Physics-Inspired Generative Models in Medical Imaging: A Review

Physics-inspired Generative Models (GMs), in particular Diffusion Models (DMs) and Poisson Flow Models (PFMs), enhance Bayesian methods and promise great utility in medical imaging. This review examines the transformative role of such generative methods. First, a variety of physics-inspired GMs, including Denoising Diffusion Probabilistic Models (DDPMs), Score-based Diffusion Models (SDMs), and Poisson Flow Generative Models (PFGMs and PFGM++), are revisited, with an emphasis on their accuracy, robustness as well as acceleration. Then, major applications of physics-inspired GMs in medical imaging are presented, comprising image reconstruction, image generation, and image analysis. Finally, future research directions are brainstormed, including unification of physics-inspired GMs, integration with Vision-Language Models (VLMs), and potential novel applications of GMs. Since the development of generative methods has been rapid, this review will hopefully give peers and learners a timely snapshot of this new family of physics-driven generative models and help capitalize their enormous potential for medical imaging.

==> content/appendices/PFGMpp.tex <==
\section*{APPENDIX B}
This appendix contains informal mathematical derivations related to PFGM++\cite{xu2023} aimed to enhance the intuition of the interested reader. As stated above, by setting  $p_r(\bm{x}|\bm{y}) \propto 1/(|| \bm{x}-\bm{y}||_2^2+r^2)^{\frac{N+D}{2}}$ we can ensure that the minimizer of Eq. \eqref{pfgmpp_obj_final} is $f^*_\theta(\bm{\tilde{x}}) = \sqrt{D} \bm{E} (\bm{\tilde{x}})_{\bm{x}} \cdot E(\bm{\tilde{x}})_r^{-1}.$ Similar to the proof of Proposition 3.2. \cite{xu2023}, this follows since the minimizer of Eq. \eqref{pfgmpp_obj_final} is 
\begin{equation}
    f^*_\theta(\bm{\tilde{x}}) = \int p_r(\bm{y}|\bm{x})\frac{\bm{x}-\bm{y}}{r/\sqrt{D}} d\bm{y} = \sqrt{D} \frac{\int p_r(\bm{x}|\bm{y})(\bm{x}-\bm{y}) p(\bm{y})d\bm{y}}{rp_r(\bm{x})}.   
    \label{pfgmpp_fstar_step1}
\end{equation}
Now, since $p_r(\bm{x}|\bm{y}) \propto 1/(|| \bm{x}-\bm{y}||_2^2+r^2)^{\frac{N+D}{2}}$ and $p_r(\bm{x})=\int p_r(\bm{x}|\bm{y})p(\bm{y})d\bm{y}$ we can rewrite the right hand side in Eq. \eqref{pfgmpp_fstar_step1} as
\begin{equation}
    \sqrt{D} \frac{\int p_r(\bm{x}|\bm{y})(\bm{x}-\bm{y}) p(\bm{y})d\bm{y}}{\int rp_r(\bm{x}|\bm{y})p(\bm{y})d\bm{y}}
    \propto \sqrt{D} \frac{\int \frac{\bm{x}-\bm{y}}{||\bm{\tilde{x}}-\bm{\tilde{y}}||^{N+D}}p(\bm{y})d\bm{y}}{\int \frac{r}{||\bm{\tilde{x}}-\bm{\tilde{y}}||^{N+D}}p(\bm{y})d\bm{y}} 
    = \sqrt{D} \bm{E} (\bm{\tilde{x}})_{\bm{x}} \cdot E(\bm{\tilde{x}})_r^{-1}.  
    \label{pfgmpp_fstar_step2}
\end{equation}

Reference \cite{xu2023} shows that both the training and sampling processes of PFGM++ converge to those of score-based diffusion models (EDM \cite{karras2022}) in the $D\rightarrow \infty, r=\sigma\sqrt{D}$ limit. To build intuition, we provide sketches of these proofs. In particular, we will start by showing that
\begin{equation}
    \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} \sqrt{D} \bm{E}(\bm{\tilde{x}})_{\bm{x}} / E(\tilde{\bm{x}})_r \propto \sigma \nabla_{\bm{x}}\log p_\sigma (\bm{x}). 
    \label{pfgmpp_obj_limit}
\end{equation}
For formal statements and proofs please see Theorem 4.1 and Proposition 4.2 in \cite{xu2023}. The limit in Eq. \eqref{pfgmpp_obj_limit} is establish by first showing that $p_r(\bm{x}|\bm{y})$ converges to $p_\sigma(\bm{x}|\bm{y})$ in the same limit. Recall that $p_r(\bm{x}|\bm{y})$ is chosen such that $p_r(\bm{x}|\bm{y}) \propto 1/(|| \bm{x}-\bm{y}||_2^2+r^2)^{\frac{N+D}{2}} = (|| \bm{x}-\bm{y}||_2^2+r^2)^{-\frac{N+D}{2}}.$ Taking the limit, we have that
\begin{align}
    \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} p_r(\bm{x}|\bm{y}) &\propto \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} (|| \bm{x}-\bm{y}||_2^2+r^2)^{-\frac{N+D}{2}} \propto \lim_{D\to \infty} \exp \left(-\frac{N+D}{2}\log (\frac{|| \bm{x}-\bm{y}||_2^2}{D\sigma^2}+1) \right) \notag \\
    &= \lim_{D\to \infty} \exp \left(-\frac{N+D}{2} \frac{|| \bm{x}-\bm{y}||_2^2}{D\sigma^2}\right) = \exp \left(-\frac{|| \bm{x}-\bm{y}||_2^2}{\sigma^2}\right) \propto p_\sigma (\bm{x}|\bm{y}). 
    \label{perturbation_limit}
\end{align}
Now, using that the right hand side in Eq. \eqref{pfgmpp_fstar_step1} is proportional to Eq. the right hand side in Eq. \eqref{pfgmpp_fstar_step2}, we establish the desired limit as 
\begin{align}
    \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} \sqrt{D} \bm{E}(\bm{\tilde{x}})_{\bm{x}} / E(\tilde{\bm{x}})_r  &\propto \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} \sqrt{D} \frac{\int p_r(\bm{x}|\bm{y})(\bm{x}-\bm{y}) p(\bm{y})d\bm{y}}{rp_r(\bm{x})} \notag \\
    &\propto \frac{\int p_\sigma(\bm{x}|\bm{y})\frac{(\bm{x}-\bm{y})}{\sigma} p(\bm{y})d\bm{y}}{p_\sigma(\bm{x})} \propto  \sigma \nabla_{\bm{x}}\log p_\sigma (\bm{x}),
\end{align}
where we used the result from Eq. \eqref{perturbation_limit} Applying a simple change-of-variables via the alignment formula $r=\sigma \sqrt{D}$, using $\sigma:=\sigma(t)=t$, yields the equivalence between $d\bm{x}/dt$ in Eq. \eqref{edm_ode} and $d\bm{x}/dr$ in Eq. \eqref{pfgmpp_ode} Finally, it is possible to show that $\lim_{D \to \infty} p_{r_{\text{max}}=\sigma_{\text{max}}\sqrt{D}} (\bm{x}) = \mathcal{N}(\bm{0},\sigma_{\text{max}}^2\bm{I}).$ Hence, the sampling process of PFGM++ converges to that of diffusion models \cite{karras2022} in the $D \to \infty, r=\sigma\sqrt{D}$ limit. To show the equivalence of the training objectives, we write the weighted denoising score matching objective for the diffusion model as
\begin{equation}
    \mathbb{E}_{\sigma \sim p(\sigma)} \mathbb{E}_{\bm{y}\sim p(\bm{y
    })} \mathbb{E}_{\bm{x}\sim p_{\sigma}(\bm{x}|\bm{y})} \left[\lambda(\sigma)||f_{\theta}(\bm{x},\sigma)-\frac{\bm{x}-\bm{y}}{\sigma}||_2^2\right]. 
    \label{edm_obj_updated}
\end{equation}
The minimizer of this objective is 
\begin{equation}
    f^*_{\theta,\text{DSM}}(\bm{x},\sigma) = \frac{\int p_\sigma(\bm{x}|\bm{y})\frac{(\bm{x}-\bm{y})}{\sigma} p(\bm{y})d\bm{y}}{p_\sigma(\bm{x})} = -\sigma \nabla_{\bm{x}}\log p_\sigma (\bm{x}). 
\end{equation}
Taking the $D \to \infty, r=\sigma \sqrt{D}$ limit
\begin{align}
    \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} f^*_{\theta,\text{PFGM++}}(\tilde{\bm{x}}) &=  \lim_{\substack{D\to \infty \\ r=\sigma \sqrt{D}}} \sqrt{D} \frac{\int p_r(\bm{x}|\bm{y})(\bm{x}-\bm{y}) p(\bm{y})d\bm{y}}{rp_r(\bm{x})} \\
    &\propto \frac{\int p_\sigma(\bm{x}|\bm{y})\frac{(\bm{x}-\bm{y})}{\sigma} p(\bm{y})d\bm{y}}{p_\sigma(\bm{x})} = f^*_{\theta,\text{DSM}}(\bm{x},\sigma),
\end{align}
where the limit is evaluated using the results from Eq. \eqref{perturbation_limit} In other words, the training objectives of diffusion models \cite{karras2022} and PFGM++ \cite{xu2023}, despite appearing widely different, are in fact equivalent in the $D \to \infty, r=\sigma \sqrt{D}$ limit. 

==> extra/authors/ar.tex <==
%Authors, affiliations address.
\author{Dennis Hein$^{1,2*}$, Afshin Bozorgpour$^{3*}$, Dorit Merhof$^{3\dag}$, Ge Wang$^{4\dag}$
\affil{$^1$Department of Physics, KTH Royal Institute of Technology,
Stockholm, Sweden.}
\affil{$^2$MedTechLabs, Karolinska University Hospital, Stockholm, Sweden.}
\affil{$^3$Faculty of Informatics and Data Science, University of Regensburg, Regensburg, Germany.}
\affil{$^4$Department of Biomedical Engineering, School of Engineering,
Biomedical Imaging Center, Center for Biotechnology and
Interdisciplinary Studies, Rensselaer Polytechnic Institute, Troy, NY,
USA.}
\affil{$^{*}$Equal contributions.}
\affil{$^{\dag}$Corresponding authors.}}


==> extra/keywords/arxiv.tex <==
Physics-inspired generative models \and
Bayesian theorem \and
%Variational Autoencoder (VAE) \and
%Generative Adversarial Network (GAN) \and
Diffusion model \and
Poisson flow generative model (PFGM)\and
PFGM++ \and 
Consistency model \and
Medical imaging \and
Image reconstruction \and
Image generation \and
Image analysis 


==> figures/methods-fig.tex <==
\begin{figure}
    \centering
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/IS3B.PNG}
        \caption{Non-Markovian generative process of I$^\text{3}$SB. From~\cite{wang2024implicit}}
        \label{fig:is-method}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/JCCS-PFGM(1).PNG}
        \caption{JCCS-PFGM framework. From~\cite{ge2023jccspfgm}}
        \label{fig:jccs-method-frame}
    \end{subfigure}\\
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/JCCS-PFGM(2)-circle-supervision.PNG}
        \caption{JCCS-PFGM's circle supervision strategy. From~\cite{wang2024implicit}}
        \label{fig:jccs-method-circle}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/JCCS-PFGM(3)-joint-connection.PNG}
        \caption{JCCS-PFGM's joint connection mechanism. From~\cite{wang2024implicit}}
        \label{fig:jccs-hoint}
    \end{subfigure}\\
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/Residual.PNG}
        \caption{Residual Denoising Diffusion Model (RDDM). From~\cite{liu2024residual}}
        \label{fig:residual}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/methods/RoentG.PNG}
        \caption{Text-to-image synthesis of chest x-ray images using RoentGen. From~\cite{chambon2022roentgen}}
        \label{fig:roent-method}
    \end{subfigure}
    
    \caption{Methods}
    \label{fig:methods}
\end{figure}

==> figures/results-fig.tex <==
\begin{figure}[H]
    \centering
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/IS3B-r1.PNG}
        \caption{CT super-resolution task results of IS$^\text{3}$. From~\cite{wang2024implicit}}
        \label{fig:is3-1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/IS3B-r2.PNG}
        \caption{Abdominal CT denoising task results of I$^\text{3}$SB. From~\cite{wang2024implicit}}
        \label{fig:is3-2}
    \end{subfigure}\\
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/JCCS-PFGM-results.PNG}
        \caption{Comparison of Low-Dose CT Reconstruction Results between JCCS-PFGM and Other Methods. From~\cite{ge2023jccspfgm}}
        \label{fig:jccs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/RoentG-synthetic-CXRs.PNG}
        \caption{Images generated by RoentGen. From~\cite{chambon2022roentgen}}
        \label{fig:roentg}
    \end{subfigure}\\
    
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/cheff-results.PNG}
        \caption{High-resolution synthetic chest X-rays produced using cascaded latent diffusion pipeline. From~\cite{weber2023cascaded}}
        \label{fig:cheff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/PS-PFCM-results.PNG}
        \caption{Comparison of Low-Dose CT Imaging: PS-PFCM (f) vs. Other Proposed Approaches}
        \label{fig:ps-pfcm}
    \end{subfigure}\\
    
    \caption{Results}
    \label{fig:Results}
\end{figure}


==> tables/landscape.tex <==
\newpage
% \begin{landscape}
\begin{sidewaystable}[!th]
    \centering
    \caption{A brief description of the reviewed Diffusion-based models in medical imaging. DD, CM, and GF respectively stand for Data Dimension, Consistency Models, GFLOPS}
    \resizebox{\textheight}{!}{
    \begin{tabular}{c|cc|cccc|c|cc|cccc}
        \toprule
        \textbf{Methodology} & \textbf{P.(M)} & \textbf{GF} & \textbf{Modality} & \textbf{DD} & \textbf{Task} & \textbf{Dataset} & \textbf{Description} & \textbf{Acceleration} & \textbf{Innovation} & \textbf{Resource} & \textbf{Inference Time} & \textbf{Sampling} & \textbf{Base Method} \\
        
        \midrule
        
        PS-PFCM & - & - & Low-dose CT & 2D & Image denoising & Mayo low-dose CT & \makecell{PS-PFCM integrates PFGMs \\ with CMs to efficiently map noise \\ to target posterior distributions, \\ significantly improving \\ image denoising performance, \\ particularly in clinical \\ low-dose CT imaging.} & - & \makecell{PS-PFCM combines PFGMs \\ and CMs for efficient image denoising} & single NVIDIA A6000 48GB & - & \makecell{Single step sampling \\ (Consistency Models)} & PFGM++ and CMs \\
        
        \midrule
        
        PPFM & - & - & Low-dose and Photon-count CT & 2D & Image denoising & \makecell{Mayo low-dose CT, \\ Photon-counting CT} & \makecell{Enhancing CT image denoising with \\ conditional generative modeling \\ and optimized PFGMs, significantly\\ reducing the Number of Function \\ Evaluations and incorporating \\ an effective regularization \\ technique for superior performance} & - & \makecell{PPFM enhances CT image denoising\\ by integrating conditional \\ generative modeling with optimized PFGMs.} & single NVIDIA A6000 48GB & - & \makecell{Single step sampling} & PFGM++ \\

        \midrule
        
        RDDM & - & - & Natural Images & 2D & \makecell{Image Generation \\ Image Restoration \\ Image Inpainting \\ image translation} & \makecell{CelebA, \\ ISTD, \\ LOL} & \makecell{Enhancing image generation and\\ restoration by splitting denoising into \\ residual and noise diffusions,\\ allowing precise control, stochastic variations,\\ and achieving SOTA performance \\with minimal training configurations.} & residual prediction & \makecell{RDDM improves image generation \\and restoration by splitting \\denoising into residual and \\noise diffusions.} & single Nvidia GTX 3090 24GB & - & \makecell{SM-Res \\ SM-N \\ SM-Res-N} & DDPM \\

        \midrule
        RoentGen & - & - & Medical Reports and CXR Images & 1D and 2D& \makecell{Text-to-image(CXR) synthesis} & \makecell{MIMIC-CXR} & \makecell{Enhancing image generation \\and restoration by splitting \\denoising into residual and\\ noise diffusions, allowing\\ precise control, stochastic variations,\\ and achieving SOTA performance\\ with minimal training configurations.} & - & \makecell{RoentGen generates high-quality,\\ synthetic chest X-rays from\\ text prompts using a \\fine-tuned latent diffusion model.} & 64 A100 GPUs & - & \makecell{-} & LDM \\
        
        \bottomrule
    \end{tabular}}
    \label{tab:comparison}
\end{sidewaystable}
% end{landscape}
\newpage

==> tables/pro.tex <==
\newpage
% \begin{landscape}
\begin{sidewaystable}[!th]
% \begin{table}[!th]
    \centering
    \caption{A brief description of the reviewed Diffusion-based models in medical imaging. DD, CM, and GF respectively stand for Data Dimension, Consistency Models, GFLOPS}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cccc|c|cc|ccc}
        \toprule
        \textbf{Methodology} & \textbf{Modality} & \textbf{DD} & \textbf{Task} & \textbf{Dataset} & \textbf{Description} & \textbf{Acceleration} & \textbf{Innovation} & \textbf{Resource} & \textbf{Sampling} & \textbf{Base Method} \\
        
        \midrule
        
        PS-PFCM & Low-dose CT & 2D & Image denoising & Mayo low-dose CT & \makecell{PS-PFCM integrates PFGMs \\ with CMs to efficiently map noise \\ to target posterior distributions, \\ significantly improving \\ image denoising performance, \\ particularly in clinical \\ low-dose CT imaging.} & - & \makecell{PS-PFCM combines PFGMs \\ and CMs for efficient image denoising} & single NVIDIA A6000 48GB  & \makecell{Single step sampling \\ (Consistency Models)} & PFGM++ and CMs \\
        
        \midrule
        
        PPFM & Low-dose and Photon-count CT & 2D & Image denoising & \makecell{Mayo low-dose CT, \\ Photon-counting CT} & \makecell{Enhancing CT image denoising with \\ conditional generative modeling \\ and optimized PFGMs, significantly\\ reducing the Number of Function \\ Evaluations and incorporating \\ an effective regularization \\ technique for superior performance} & - & \makecell{PPFM enhances CT image denoising\\ by integrating conditional \\ generative modeling with optimized PFGMs.} & single NVIDIA A6000 48GB & \makecell{Single step sampling} & PFGM++ \\

        \midrule
        
        RDDM  & Natural Images & 2D & \makecell{Image Generation \\ Image Restoration \\ Image Inpaiting \\ image translation} & \makecell{CelebA, \\ ISTD, \\ LOL} & \makecell{Enhancing image generation and\\ restoration by splitting denoising into \\ residual and noise diffusions,\\ allowing precise control, stochastic variations,\\ and achieving SOTA performance \\with minimal training configurations.} & residual prediction & \makecell{RDDM improves image generation \\and restoration by splitting \\denoising into residual and \\noise diffusions.} & single Nvidia GTX 3090 24GB & \makecell{SM-Res \\ SM-N \\ SM-Res-N} & DDPM \\

        \midrule
        RoentGen  & Medical Reports and CXR Images & 1D and 2D& \makecell{Text-to-image(CXR) synthesis} & \makecell{MIMIC-CXR} & \makecell{RoentGen is a vision-language model\\ generating synthetic chest X-rays\\ from text prompts by fine-tuning\\ a latent diffusion model,\\ improving image classification\\ but facing challenges like\\ dataset reliance and potential overfitting.} & - & \makecell{RoentGen generates high-quality,\\ synthetic chest X-rays from\\ text prompts using a \\fine-tuned latent diffusion model.} & 64 A100 GPUs & \makecell{-} & LDM \\

        \midrule
        JCCS-PFGM & \makecell{Multiphase contrast-enhanced\\ computed tomography (CECT)} & 1D and 2D& \makecell{Image Reconstruction} & \makecell{Private} & \makecell{JCCS-PFGM enhances multiphase CECT image quality\\ and reduces radiation exposure using progressive\\ low-dose reconstruction, circle-supervision, and \\joint condition mechanisms. It optimizes radiation dosage\\ and image clarity by leveraging temporal progression and spatial correlations.} & - & \makecell{JCCS-PFGM enhances multiphase CECT image quality\\ and reduces radiation exposure\\ using progressive low-dose reconstruction,\\ circle-supervision,\\ and joint condition mechanisms.} &- & \makecell{Circle-supervision strategy strategy} & \makecell{PFGM} \\

        \midrule
        QSMDiff  & MRI & 3D & \makecell{Quantitative Susceptibility\\ Mapping} & COSMOS & \makecell{QSMDiff is a 3D diffusion model\\ for MRI Quantitative Susceptibility Mapping\\ that enhances image quality and \\efficiency by using unsupervised\\ 3D image patch training and\\ measurement-guided inference.} & - & \makecell{The paper introduces QSMDiff,\\ a groundbreaking 3D image patch-based\\ diffusion model for robustly handling MRI\\ Quantitative Susceptibility Mapping,\\ offering super-resolution\\ and image denoising capabilities.} & \makecell{Single Nvidia H100 GPU (80GB) \\ Single RTX 4090 GPU (24GB)}& conditional sampling & \makecell{patch-based DDPM} \\

        \midrule
        Hyper-Diffusion  & \makecell{CT-Scan \\ Natural Image} & 2D & \makecell{CT reconstriction \\ Weather forecasting} & \makecell{LUNA \\  ERA5} & \makecell{HyperDiffusion combines conditional denoising diffusion models\\ and hyper-networks to enhance predictive\\ capabilities by estimating and \\disentangling epistemic and aleatoric \\uncertainties, outperforming\\traditional methods in applications like medical imaging.} & - & \makecell{HyperDiffusion introduces a method combining\\ conditional denoising diffusion models\\ and hyper-networks to estimate and\\ disentangle epistemic and aleatoric uncertainties.} &  single NVIDIA RTX A6000 & \makecell{Hypernetworks} & DDPM \\

        \midrule
        MAEDiff & MRI & 3D & \makecell{Unsupervised anomaly detection} & \makecell{IXI \\ BraTS21 \\ MSLUB} & \makecell{MAEDiff is a Masked Autoencoder-enhanced Diffusion Model\\ designed for unsupervised anomaly detection\\ in brain images, employing a hierarchical\\ patch partitioning strategy to improve\\ focus on unnoised regions and enhance\\ image reconstruction quality.} & - & \makecell{MAEDiff introduces a Masked Autoencoder-enhanced\\ Diffusion Model for superior \\unsupervised anomaly detection in brain images.} & single NVIDIA GeForce RTX 3090 GPU (24GB) & \makecell{Patch-based$^*$} & \makecell{MAE \\ DDPM} \\

        \midrule
        BerDiff  & \makecell{CT \\ MRI} & 2D & \makecell{Medical Image Segmentation} & \makecell{LIDC-IDRI \\ BRATS 2021} & \makecell{BerDiff enhances traditional diffusion methods \\for medical image segmentation by incorporating\\ Bernoulli noise, resulting in more accurate \\and diverse segmentation masks, especially for ambiguous tumor boundaries.} & - & \makecell{The incorporation of Bernoulli noise\\ into diffusion methods, enhancing \\the accuracy and diversity of segmentation masks \\for binary tasks in medical imaging.} & single NVIDIA V100& Bernoulli & \makecell{DDPM \\ DDIM} \\

        \midrule
        MedSegDiff-V2  & \makecell{CT \\ MRI \\ Ultrasound \\ Dermographic} & \makecell{2D}& \makecell{Medical Image Segmentation} & \makecell{AMOS2022 \\ BTCV \\ REFUGE-2 \\ BraTs-2021 \\ ISIC 2018 \\ TNMIX} &  \makecell{integrating ViT into a DPM \\  to enhance the accuracy and \\ diversity of medical image segmentation,\\ using innovative conditioning approaches \\ like Anchor Condition and Semantic Condition.} & - & \makecell{Introducing ViT and novel conditioning approaches,\\ such as the Anchor Condition and Semantic Condition} & 4 NVIDIA A100 GPU& - & DPM \\

        \midrule
        VALD-MD   & X-ray & 2D & \makecell{Anomaly Detection} & \makecell{COVID-19 Radiography Database} &  \makecell{Proposing a method that uses latent diffusion\\ models and domain-specific language models\\ to generate "normal counterparts" \\for abnormal medical images, \\enhancing interpretability and explainability in disease detection.} & - & \makecell{Producing visual attribution maps \\highlighting diagnostically relevant differences\\ and 
        Enhancing explainability in disease detection.} & single Quadro RTX 8000& - & LDM \\

        \midrule
        LeFusion  & MRI & 2D & \makecell{Cardiac MRI synthesis} & \makecell{EMIDEC} & \makecell{Introducing a lesion-focused diffusion model \\that addresses long-tail imbalance and algorithmic unfairness\\ in clinical data by enhancing lesion \\synthesis and maintaining background quality.} & - & \makecell{Integrating forward-diffused background contexts,\\ handling multi-class lesions with diverse\\ masks, and using a 3D U-Net for lesion-focused denoising} & -& DM & \makecell{DM\\ nnUNet} \\

        \midrule
        Unconditional LDM  & \makecell{X-ray \\ MRI \\ PCCTA} & \makecell{2D \\ 3D}& \makecell{-} & \makecell{Chestx-ray8 \\ Knee-MRI \\ Photon counting CT Angiography\\ (Private)} & \makecell{Identifying influential factors and\\ employing a composite loss function\\ and contrastive learning to enhance\\ image generation and differentiation.} & - & \makecell{Exploring key memorization factors,\\ using a composite loss function,\\ deploying contrastive learning for\\ novel image differentiation,\\ and advocating for memorization-aware metrics\\ and differential privacy.} & - & - & LDM \\
        
        \midrule
        THOR   & \makecell{MRI} & \makecell{2D}&  \makecell{Anomaly Detection}& \makecell{IXI \\ Atlas V2.0} & \makecell{A novel diffusion model approach for\\ enhancing unsupervised anomaly detection \\in medical imaging by using temporal\\ anomaly maps to guide the denoising process} & - & \makecell{leveraging intermediate anomaly maps and \\a blending process to preserve healthy tissue\\ integrity while minimizing anomalies, improving\\ specificity and reliability in medical diagnostics} & - & - & DDPM \\

        \midrule
        Cheff  & \makecell{X-ray \\ Clinical reports} & \makecell{2D \\ 1D}& \makecell{Medical Image Synthesis} & \makecell{ChestX-ray14 \\ CheXpert \\ MIMIC-CXR \\ PadChest \\ BRAX \\ VinDr-CXR} & \makecell{Introducing a cascaded latent diffusion model, \\generating high-quality chest radiographs,\\ and MaCheX, a large chest X-ray dataset.\\ Cheff explores report-to-chest-X-ray generation,\\ aiming to improve medical AI assistance.} & - & \makecell{Setting new standards in radiological image synthesis\\ and advancing medical AI with publicly \\accessible models and data.} & 8 A100 & - & LDM \\

        \midrule
        U$^2$MRPD  & \makecell{MRI} & \makecell{2D}& \makecell{Image Reconstruction}& \makecell{IXI \\ FastMRI} & \makecell{Proposing the Unsupervised Undersampled MRI Reconstruction \\by Prompting a pre-trained latent Diffusion model,\\ leveraging large latent diffusion models trained on \\natural images for medical imaging applications.} & - & \makecell{Leveraging LLDMs for unsupervised MRI reconstruction,\\ showcasing superior adaptability and generalizability \\without specific medical image training,\\ marking a significant advancement in medical imaging.} & Single 3090 GPU & - & LDM \\

        % \midrule
        % U$^2$MRPD  & - & -& - & - & - & - & - & & - & - \\

        \midrule
        SDPS   & CT & \makecell{2D}& \makecell{Medical Image Reconstruction} & \makecell{-} & \makecell{applying diffusion models to spectral CT reconstruction,\\ improving image quality by synergistically reconstructing\\ multiple images across different energy bins.} & - & \makecell{Introducing Plain Diffusion Posterior Sampling (PDPS) \\and Spectral DPS (SDPS), utilizing denoising diffusion models \\to address inverse problems in medical imaging,\\ enhancing image quality and managing noise in spectral CT.} & RTX 2080 Ti & Posterior Sampling & DDPM \\

        \midrule
        I$^3$SB  & \makecell{CT} & 2D & \makecell{Super Resolution \\ Denoising} & \makecell{RPLHR-CT} & \makecell{Introducing the Implicit Image-to-Image Schrödinger Bridge (I$^3$SB),\\ improving upon the Image-to-Image Schrödinger Bridge (I$^2$SB)\\ by incorporating a non-Markovian process.} & - & \makecell{Adjusting the generative process to include \\the initial corrupted image at each step,\\ improving texture restoration and expediting image generation,\\ offering a robust framework for medical imaging applications.} & - & - & I$^2$SB \\

        \midrule
        Unsupervised PPFM & CT & 2D & \makecell{Medical Image Denoising} & \makecell{Mayo low-dose CT \\ Photon-counting CT} & \makecell{Introducing the Posterior Sampling Poisson\\ Flow Generative Models (PPFM), refining\\ the PFGM++ for efficient denoising of\\ low-dose and photon-counting CT images.} & - & \makecell{PPFM transitions from unconditional to conditional generation,\\ incorporating the condition image into the process,\\ accelerating sampling, and applying a simple\\ regularization technique for improved denoising.} & A6000 48GB GPU & - & PFGM++ \\
        \midrule
        
        CTS  & \makecell{MRI \\ Ultrasound} & 2D & \makecell{Medical Image Segmentation} & \makecell{BRATS2021 \\ SEPHI} & \makecell{CTS leverages consistency models \\for efficient medical image segmentation \\motivated by addressing the struggling of\\ DMs in slow predictions.} & - & \makecell{CTS reduces time consumption by\\ transforming multiple samplings into one,\\ improving segmentation with a joint\\ loss function and multi-scale \\feature supervision, showcasing the potential of\\ consistency models in medical imaging.} & GTX 4090 & - & CT \\
        \midrule
        
        VM-DDPM  & \makecell{MRI\\ X-ray} & 2D & \makecell{Medical Image Synthesis} & \makecell{ACDC \\ BRATS2018 \\ ChestXRay} & \makecell{Proposing the VM-DDPM for medical image synthesis,\\ combining CNN's local perception with the SSM\\ for global modeling, maintaining structural\\ texture consistency with linear computational complexity.} & - & \makecell{Combining CNN and SSM for medical image synthesis,\\ ensuring structural texture consistency\\ while maintaining linear computational complexity.} & GeForce RTX 4090 GPU & - & \makecell{VMamba \\ DDPM} \\
        \midrule
        
        WDM  & MRI & 3D & \makecell{Medical Image Enhancement} & \makecell{BRATS-2023 \\ MS} & \makecell{Pseudo-3D models have enhanced diffusion models\\ for MR image denoising, outperforming traditional\\ methods like FSL in brain tissue segmentation.} & - & - & & - & - \\
        \bottomrule
    \end{tabular}}
    \label{tab:comparison}
% \end{table}
\end{sidewaystable}
% \end{landscape}

